Duet: Creating Harmony between Processors and Embedded FPGAs

The demise of Moore's Law has led to the rise of hardware acceleration. However, the focus on accelerating stable algorithms in their entirety neglects the abundant fine-grained acceleration opportunities available in broader domains and squanders host processors' compute power. This paper presents Duet, a scalable, manycore-FPGA architecture that promotes embedded FPGAs (eFPGA) to be equal peers with processors through non-intrusive, bi-directionally cache-coherent integration. In contrast to existing CPU-FPGA hybrid systems in which the processors play a supportive role, Duet unleashes the full potential of both the processors and the eFPGAs with two classes of post-fabrication enhancements: fine-grained acceleration, which partitions an application into small tasks and offloads the frequently-invoked, compute-intensive ones onto various small accelerators, leveraging the processors to handle dynamic control flow and less accelerable tasks; hardware augmentation, which employs eFPGA-emulated hardware widgets to improve processor efficiency or mitigate software overheads in certain execution models. An RTL-level implementation of Duet is developed to evaluate the architecture with high fidelity. Experiments using synthetic benchmarks show that Duet can reduce the processor-accelerator communication latency by up to 82% and increase the bandwidth by up to 9.5x. The RTL implementation is further evaluated with seven application benchmarks, achieving 1.5-24.9x speedup.

==> figures/sorting_example.tex <==
\begin{figure}[t!]
    
    \centering

    \begin{subfigure}[t]{0.53\linewidth}
        \centering
        \includegraphics[trim=0pt 4pt 0pt 3pt, clip, width=\linewidth]{images/sorting_acc.pdf}
        \setlength{\abovecaptionskip}{-8pt}
        \setlength{\belowcaptionskip}{-4pt}
        % \caption{Block Diagram of an 8-Element Bitonic Sorting Accelerator}
        \caption{}
        \label{fig:sorting-acc}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.42\linewidth}
        \centering
        \includegraphics[trim=0pt 4pt 0pt 3pt, clip, width=\linewidth]{images/sorting_timing.pdf}
        \setlength{\abovecaptionskip}{-8pt}
        \setlength{\belowcaptionskip}{-4pt}
        % \caption{Timeline of the Processor and a 33-Element Bitonic Sorting Accelerator Cooperatively Sorting a 70-Element Array}
        \caption{}
        \label{fig:sorting-timeline}
    \end{subfigure}
    
    % \setlength{\belowcaptionskip}{-12pt}
    \setlength{\abovecaptionskip}{4pt}
    \caption{Bitonic Sorting Accelerator}
    
    \begin{FlushLeft}
    \fontsize{9}{10}\selectfont
    \vspace{-0.6\baselineskip}
    (a) Block diagram of a bitonic sorting accelerator.
    Each pair of dots connected with a vertical line represents a compare-and-swap operation.
    (b) Timeline of a processor and a 32-element bitonic sorting accelerator cooperatively sorting a 70-element array.
    \vspace{-1.5\baselineskip}
    \end{FlushLeft}
    
    \label{fig:sorting-example}
    
\end{figure}

==> tables/area.copy.tex <==
\begin{table}[t]

    \small
    \setlength\tabcolsep{2pt}
    \centering
    \newcounter{notenumber}
    \newcommand{\mynote}{\textsuperscript{\fnsymbol{notenumber}}}
    \newcommand{\newnote}{\stepcounter{notenumber}\mynote{}}

        % \setlength{\belowcaptionskip}{-8pt}
        \caption{\centering
        Area and Typical Frequency of Dolly Components}
        
    \begin{threeparttable}[t]
        \begin{tabular}{|c|c|c|c|}
        
        \hline
        
        % title row (upper half)
        \multirow{2}{*}{Component} &
        Device &
        Area &
        Max. Frequency \\
        
        % title row (lower half)
        &
        Technology &
        ($mm^2$) &
        ($MHz$) \\
        
        \hline \hline
        
        % ariane row (upper half)
        \multirow{2}{*}{Ariane~\cite{ariane-area}} &
        GlobalFoundries &
        \multirow{2}{*}{0.39 (\textbf{1.56}\newnote{})} &
        \multirow{2}{*}{910 (\textbf{455}\mynote{})} \\
        
        % ariane row (lower half)
        &
        22$nm$ FDX &
        &
        \\
        
        \hline
        
        % p-mesh row (upper half)
        P-Mesh &
        \multirow{2}{*}{IBM~32$nm$~SOI} &
        \multirow{2}{*}{0.55 (\textbf{1.1}\mynote{})} &
        \multirow{2}{*}{1000 (\textbf{711}\mynote{})} \\
        
        % p-mesh row (lower half)
        Socket~\cite{openpiton} &
        &
        &
        \\
        
        \hline
        
        % control tile row (upper half)
        FPGA~Mgr~+ &
        \multirow{4}{*}{FreePDK45} &
        \multirow{2}{*}{0.21} &
        \multirow{2}{*}{925} \\
        
        % control tile row (lower half)
        Soft~Reg~Intf &
        &
        &
        \\
        
        \cline{1-1} \cline{3-4}
        
        % memory tile row (upper half)
        Coherent &
        &
        \multirow{2}{*}{0.04} &
        \multirow{2}{*}{1250} \\
        
        % memory tile row (lower half)
        Memory Intf &
        &
        &
        \\
        
        % \hline
        
        % fpga row (upper half)
        % FPGA~Sub- &
        % \multirow{2}{*}{40$nm$} &
        % \multirow{2}{*}{-} &
        % \multirow{2}{*}{-} &
        % \multirow{2}{*}{-} &
        % \multirow{2}{*}{-} \\
        
        % fpga row (lower half)
        % Array~\cite{vtr}\newnote{} &
        % &
        % &
        % &
        % &
        % \\
        
        \hline
        \end{tabular}
        
        \setcounter{notenumber}{0}
        
        \begin{tablenotes}
            \item [\stepcounter{notenumber}\fnsymbol{notenumber}] \fontsize{9}{9}\selectfont Scaled down to 45$nm$ with a linear MOSFET scaling model
            % \item [\stepcounter{notenumber}\fnsymbol{notenumber}] \footnotesize Miscellaneous components in a physical tile
            % \item [\stepcounter{notenumber}\fnsymbol{notenumber}] \footnotesize See Sec.~\ref{sec:eval-arch}
        \end{tablenotes}
        
        \vspace{-1.2\baselineskip}
        
    \end{threeparttable}
    \label{tab:area}

\end{table}
